Active Covering

We analyze the problem of active covering, where the learner is given an unlabeled dataset and can sequentially label query examples. The objective is to label query all of the positive examples in the fewest number of total label queries. We show under standard non-parametric assumptions that a classical support estimator can be repurposed as an offline algorithm attaining an excess query cost of $\widetilde{\Theta}(n^{D/(D+1)})$ compared to the optimal learner, where $n$ is the number of datapoints and $D$ is the dimension. We then provide a simple active learning method that attains an improved excess query cost of $\widetilde{O}(n^{(D-1)/D})$. Furthermore, the proposed algorithms only require access to the positive labeled examples, which in certain settings provides additional computational and privacy benefits. Finally, we show that the active learning method consistently outperforms offline methods as well as a variety of baselines on a wide range of benchmark image-based datasets.

==> UCB.tex <==
\section{Active UCB Learner}\label{sec:ucb}

\begin{algorithm}[t]
   \caption{Active UCB Learner}
   \label{alg:active_ucb}
\begin{algorithmic}
   \STATE {\bf Inputs}: Dataset $X$, initial sample size $m$, $\sigma$.
   \STATE Let $X_0$ be $m$ examples sampled uniformly without replacement from $X$.
   \STATE Label query $X_0$ and let $X_{+, 0}$ be the positive examples.
   \STATE Initialize $X_p \leftarrow X_{+, 0}$ and $X_a \leftarrow X_0$.
   \STATE Initialize active set \begin{align}\label{eqn:active}
       \mathcal{A} \leftarrow \left(\bigcup_{x \in X_p} B\left(x, \sigma \cdot \left(\frac{\log^2 |X_p|}{|X_p|}\right)^{1/D}\right)  \right).
   \end{align}
   \WHILE{not all positives examples in $X$ are labeled}
   \STATE Label query uniformly sampled $x \in \mathcal{A} \cap (X \backslash X_a)$.
   \IF{$x$ has a positive label}
   \STATE $X_p \leftarrow X_p \cup \{ x \}$.
   \STATE Update $\mathcal{A}$ as per (\ref{eqn:active}) with the updated $X_p$.
   \ENDIF
   \STATE $X_a \leftarrow X_a \cup \{ x \}$.
   \ENDWHILE
\end{algorithmic}
\end{algorithm}

In this section, we propose and analyze the Active UCB Learner (Algorithm~\ref{alg:active_ucb}). It proceeds by first sampling $m$ examples to label query and then throughout the algorithm, it maintains an active set $\mathcal{A}$, which when the hyperparameter $\sigma$ is sufficiently large, will satisfy the property that $\X_+ \subseteq \mathcal{A}$ and that $\mathcal{A} \rightarrow \X_+$ as the algorithm labels more positive examples, as we will show later. Thus, this strategy resembles an Upper Confidence Bound (UCB)-type approach since it maintains an upper estimate of $\X_+$ (as opposed to in the classical setting where it maintains an upper estimate of a scalar value), and the $\sigma$ is analogous to scaling the confidence band.

Algorithm~\ref{alg:active_ucb} can be seen as using a similar support estimation strategy as the offline learner, but it actively updates the positive support estimator making it tighter after each positive example queried, whereas in the offline learner, it's fixed based on the initial sample.
%\todo{The while statement in Alg 2 is not testable in practice. Is there a bound we can provide on the number of iterations we need before the condition is met (with high probability)? Or at the very least, can mention in practice, we stop when enough positive examples are found, where ``enough'' is an parameter of the task that is known a priori.} 

We now analyze the procedure, with details located in the Appendix. There are three key steps. First, we show that for $\sigma$ sufficiently large, $\X_+ \subseteq \mathcal{A} \subseteq B(\X_+,\epsilon)$ for appropriately chosen $\epsilon$. Second, we justify that this $\epsilon$ decreases at a certain rate. Finally, we combine these two results to show the following excess query cost guarantee.

\begin{theorem}[Excess Query Cost for Active UCB Learner]\label{theorem:ucb}
Suppose that Assumptions~\ref{a1},~\ref{a2}, and~\ref{a3} hold. There exists $C, \sigma_0, M_0 > 0$ depending only on $\mathcal{P}$ such that the following holds.
Let $0 < \delta < 1$ and suppose that $\sigma \ge \left(\sigma_0 \log(4n/\delta)\right)^{1/D}$
and $\frac{m}{\log^2 m}  \ge \max \left\{M_0\log(4/\delta), \frac{2\log(4/\delta)}{p^2}\right\}$ in Algorithm~\ref{alg:active_ucb}.
Then with probability at least $1-\delta$:
\begin{align*}
    E[C_{\text{ucb}}]\le (1-p)\cdot m + C \cdot \sigma \cdot \log^2 n\cdot  n^{(D-1)/D}.
\end{align*}
\end{theorem}
We see that we have a faster rate of $\widetilde{O}(n^{(D-1)/D})$ compared to the rate of $\widetilde{\Theta}(n^{D/(D+1)})$ for offline.
It's worth nothing that the active UCB algorithm has an additional hyperparameter $\sigma$ (in addition to the initial sample size $m$), which may make it more difficult to use in practice. The next active learning procedure we show will not have any additional hyperparameters.



\subsection{Proofs for Section~\ref{sec:ucb}}


We first give the result that throughout the algorithm, the active set $\mathcal{A}$ in Algorithm~\ref{alg:active_ucb} indeed satisfies the properties of an upper-confidence estimate of $\X_+$, namely that it both covers $\X_+$ and does not over-cover $\X_+$ by more than $\epsilon$, thus also making it an accurate cover.
\begin{lemma}\label{lemma:ucb_active_set}
Suppose that Assumptions~\ref{a1},~\ref{a2}, and~\ref{a3} hold.
Let $0 < \delta < 1$ and suppose that $\sigma$ and $|X_p|$ in Algorithm~\ref{alg:active_ucb} at all times satisfies
\begin{align*}
    \sigma \ge \left(\frac{C_0\cdot D \log(2n/\delta)}{\lambda_0 \cdot C_+ \cdot v_D}\right)^{1/D}, \hspace{0.5cm} \frac{|X_p|}{\log^2 |X_p|}  \ge \frac{C_0\cdot D\log(2/\delta)}{\min\{r_0, r_1\}^D\cdot \lambda_0\cdot C_+\cdot v_D}.
\end{align*}
Then
we have that with probability at least $1-\delta$, the following holds uniformly at all times in Algorithm~\ref{alg:active_ucb}:
\begin{align*}
    \X_+ \subseteq \mathcal{A} \subseteq B(\X_+, \epsilon),
\end{align*}
where $\epsilon := \sigma\cdot \big(\log^2 (|X_p|)/|X_p|\big)^{1/D}$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:ucb_active_set}]
Since $X_p \subseteq \X_+$, we have $\mathcal{A} \subseteq B(\X_+, \epsilon)$.
It thus suffices to show that for each $x \in \X_+$, there exists an example in $X_p$ within $\epsilon$ of $x$.
By the conditions on $\sigma$ and $X_p$, we have that for all $x \in \X_+$
\begin{align*}
    \mathcal{P}_+(B(x, \epsilon)) &\ge \lambda_0 \cdot C_+ \cdot v_D\cdot \epsilon^D \ge \frac{C_0\cdot D\log(2n/\delta) \log(|X_p|)}{|X_p|}.
\end{align*}
We have using Lemma~\ref{lemma:ball_bound} that with probability at least $1 - \delta/n$ uniformly in $x\in \X_+$ that the previous implies that $X_p \cap B(x, \epsilon)$ is non-empty. Therefore, $\X_+ \subseteq \mathcal{A}$.

The result follows by applying union bound across all iterations of the algorithm.
\end{proof}


Note that throughout, the value of $\epsilon$ will determine the expected excess query cost for our analysis because the excess label queries are precisely points that are chosen to be labeled queried that are in the active set $\mathcal{A}$ but outside of $\X_+$ and therefore are in the $\epsilon$-radius tube around $\X_+$. Based on Lemma~\ref{lemma:ucb_active_set}, the value of epsilon only depends on the number of positive examples queried thus far (as well as a $\log(n/\delta)$ dependence for a union bound argument leading to a high probability $1-\delta$ guarantee). We therefore now show that the number of positive examples increases at a certain rate (and thus $\epsilon$ would decrease at a certain rate).

Let $T_{\text{ucb}}(\ell)$ be the random variable for the number of iterations in Algorithm~\ref{alg:active_ucb} for which the number of positive examples queried so far is $\ell$. $T_{\text{ucb}}(\ell)$ is thus the interval of time for which $|X_p| = \ell$, and it is also the number of time steps required to sample the ($\ell$+1)-th positive example starting from $\ell$ positive examples.

Let $T_{\text{opt}}(\ell)$ be the same but for the optimal learner which labels examples uniformly from $X \cap \X_+$. We now show the following result which bounds the expected time:
\begin{lemma}\label{lemma:stopping_time}
Suppose that the conditions of Lemma~\ref{lemma:ucb_active_set} hold. Let $n_+$ be the random variable for the total number of positive examples.
Then the following is true for any $\ell := |X_p| < n_+$ throughout Algorithm~\ref{alg:active_ucb} for some $C > 0$ depending on $\mathcal{P}$:
\begin{align*}
   \E[T_{\text{ucb}}(\ell)]  -  \E[T_{\text{opt}}(\ell)] \le C \cdot \sigma \cdot n \cdot \E_{n_+} \left[ \frac{ (\log^2 (\ell) / \ell)^{1/D}}{n_+ - \ell + 1} \right],
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:stopping_time}]
Let us denote $\mathcal{A}(t)$, $X_a(t)$ and $X_p(t)$ to be the values of $\mathcal{A}$, $X_a$ and $X_p$, respectively, after the $t$-th query. Let us also denote
$\epsilon(\ell) := \sigma \cdot (\log^2 \ell / \ell)^{1/D}$.
Let $t_\ell$ be the smallest $t_\ell$ such that $|X_p(t_\ell)| =\ell$.

We have $\E[T_{\text{ucb}}(\ell) | X_a(t_\ell)]$ is the expected number of points we have to query before we query a positive example.
At each time step from $t_\ell$, until we label query a positive example, we sample uniformly from the set of unlabeled points in $\cup_{x\in X_p(t_\ell)}B(x, \epsilon(\ell))$, There are three cases:
\begin{itemize}
    \item We sample a positive example in $\X_+$.
    \item We sample a negative example in $\X_+$.
    \item We sample a negative example in $\mathcal{A}(t_\ell) \backslash \X_+$.
\end{itemize}
We repeatedly sample until the first event happens.
Let the total number of such unlabeled examples at time $t_\ell$ for each of the three above cases be $P$, $Q$, and $R$, respectively.
By Theorem 2.5 of \cite{ahlgren2014probability} (since this is the problem of expected number of draw without replacement until first success) we have
\begin{align*}
    \E[T_{\text{ucb}}(\ell) | X_a(t_\ell)] = \mathbb{E}\left[ \frac{P + Q + R + 1}{P + 1}|  X_a(t_\ell) \right]
\end{align*}
Similarly, we have
\begin{align*}
     \E[T_{\text{opt}}(\ell) | X_a(t_\ell)] = \mathbb{E}\left[ \frac{P + Q + 1}{P + 1}|  X_a(t_\ell) \right]
\end{align*}
since it's the same situation except the last situation never happens.
Therefore,
\begin{align*}
    \E[T_{\text{ucb}}(\ell) | X_a(t_\ell)]  -  \E[T_{\text{opt}}(\ell) | X_a(t_\ell)] \le \E \left[\frac{R}{P+1} | X_a(t_\ell) \right] = \E \left[ \frac{R}{n_+ - \ell + 1} | X_a(t_\ell) \right],
\end{align*}
where $n_+$ is the total number of positive examples.
Therefore, computing the expectation of both sides with respect to $X_a(t_\ell)$ gives
\begin{align*}
    \E[T_{\text{ucb}}(\ell)]  -  \E[T_{\text{opt}}(\ell)] \le \E \left[ \frac{R}{n_+ - \ell + 1} \right],
\end{align*}

We note that by Lemmas~\ref{lemma:volume} and~\ref{lemma:ucb_active_set}, the probability of labeling an example in $\mathcal{A}(t_\ell)\backslash \X_+$ is at most $C_+'\cdot \epsilon(\ell)$. This gives us:
\begin{align*}
   \E[T_{\text{ucb}}(\ell)]  -  \E[T_{\text{opt}}(\ell)] \le \E_{n_+} \left[ \frac{C \cdot \sigma \cdot (\log^2 (\ell) / \ell)^{1/D}\cdot n}{n_+ - \ell + 1} \right],
\end{align*}
as desired.
\end{proof}
We now combine Lemma~\ref{lemma:ucb_active_set} and~\ref{lemma:stopping_time} and provide the excess query cost guarantee on Algorithm~\ref{alg:active_ucb}.

\begin{proof}[Proof of Theorem~\ref{theorem:ucb}]
Take
\begin{align*}
    \sigma_0 = \frac{C_0\cdot D}{\lambda_0 \cdot C_+ \cdot v_D}, \hspace{0.5cm} M_0 = \frac{2C_0\cdot D\log(4/\delta) \min\{r_0, r_1\}^{-D}}{p\cdot \lambda_0\cdot C_+\cdot v_D}.
\end{align*}

Suppose that the total number of positive examples is $n_+$ and the number of positive examples in the initially sampled $m$ points is $m_+$.
We have with probability at least $1-\delta/2$ by Hoeffding's inequality that $m_+ \ge mp/2$ based on the condition on $m$. Then, by the condition on $m$, we also have that $m_+$ is sufficiently large for the earlier Lemmas to hold.
We see that:
\begin{align*}
    E[C_{\text{ucb}}]
    &= (1-p)\cdot m + \E_{n_+,m_+}\left[\sum_{\ell=m_+}^{n^+} E[T_{\text{ucb}}(\ell)] - E[T_{\text{opt}}(\ell)]\right] \\
    &\le (1-p)\cdot m + \sum_{\ell=1}^{n} \sigma  \cdot C_1 \cdot \left(\frac{\log^2 \ell}{\ell}\right)^{1/D}
    \cdot E[T_{\text{opt}}(\ell)],\\
    &\le (1-p)\cdot m + C_2\cdot \sigma  \sum_{\ell=1}^{n}\left(\frac{\log^2 \ell}{\ell}\right)^{1/D}\\
    &\le (1-p)\cdot m + C_2 \cdot \sigma  \log^2 n \cdot \sum_{\ell=1}^{n}\left(\frac{1}{\ell}\right)^{1/D}\\
    &\le (1-p)\cdot m + C \cdot \sigma \log^2 n \cdot n^{(D-1)/D}.
\end{align*}
where the first inequality holds for some $C_1$ because of Lemma~\ref{lemma:stopping_time}, the second inequality holds for some $C_2$ because $E[T_{\text{opt}}(\ell)]$ can be upper bounded by a constant depending on $\mathcal{P}$, and the last inequality holds for some $C$ by
\cite{chlebus2009approximate} which gives an upper bound for the sum of a $p$-series. $C_1,C_2,C$ all only depend on $\mathcal{P}$.
\end{proof}
